ResiLogic: Leveraging Composability and Diversity to Design Fault and Intrusion Resilient Chips

A long-standing challenge is the design of chips resilient to faults and glitches. Both fine-grained gate diversity and coarse-grained modular redundancy have been used in the past. However, these approaches have not been well-studied under other threat models where some stakeholders in the supply chain are untrusted. Increasing digital sovereignty tensions raise concerns regarding the use of foreign off-the-shelf tools and IPs, or off-sourcing fabrication, driving research into the design of resilient chips under this threat model. This paper addresses a threat model considering three pertinent attacks to resilience: distribution, zonal, and compound attacks. To mitigate these attacks, we introduce the \texttt{ResiLogic} framework that exploits \textit{Diversity by Composability}: constructing diverse circuits composed of smaller diverse ones by design. This gives designer the capability to create circuits at design time without requiring extra redundancy in space or cost. Using this approach at different levels of granularity is shown to improve the resilience of circuit design in \texttt{ResiLogic} against the three considered attacks by a factor of five. Additionally, we also make a case to show how E-Graphs can be utilized to generate diverse circuits under given rewrite rules.

==> eval-strategy.tex <==
\section{CMF Compute Engine}
\label{sec:eval-strategy}
We implemented a CMF Compute Engine to use as our evaluation testbed.
% We plan to make this tool (implemented in \textit{Perl} and  \textit{Verilog}) publicly available for the research community.
To the best of our knowledge, there are two previous works that 
% focus on how to 
quantify diversity in order to build fault tolerant redundant systems. Mitra et. al.~\cite{mitra2004efficient} proposed fault injection at the gate level to  compute if both designs produce same type of erroneous output, resulting in a CMF. This method is based on simulation and provides a reliability measure of the design in case of random faults.
However, to capture true CMFs, identical faults must be injected in redundant designs followed by fault simulation.
The work in~\cite{alcaide2017dimp, babu2019efficient} accelerate the diversity metric computation by analyzing circuit paths of gate level netlists of designs. The aim of the proposed tool is to measure the rate of CMF among redundant designs, therefore, a variant of the approach proposed in~\cite{mitra2004efficient} is employed to cater for the need to inject identical faults. 

\subsection{Architecture}
Fig.~\ref{fig:cmf-compute-engine} shows the block diagram of the proposed common mode failure computing engine. It fetches a set of diverse replicas from the library generated by the method discussed in Section~\ref{sec:resilogic-framework}.
No fault is injected in $RR$, which serves as a reference circuit producing the golden output. 
The number and sites of faults to be injected depends on the selected fault campaign as discussed in Section~\ref{sec:attack-model}.
Eqn.~\ref{eqn:cmf-det} shows that for the CMF output to be true, all outputs from the replicas must be equal to each other and different from the reference output $RO$: 

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/cmf-engine.pdf}
    \caption{CMF Computing Engine Architecture.}
    \label{fig:cmf-compute-engine}
\end{figure}

\begin{equation}
\label{eqn:cmf-det}
    CMF \equiv O_i=O_j \quad AND \quad O_1 \neq RO \quad \forall\ i \neq j
\end{equation}

The CMF detector in Fig.~\ref{fig:cmf-compute-engine} implements Eqn.~\ref{eqn:cmf-det} and its output is either $1$ or $0$. The aggregator stores and provides statistics for CMF results against different fault campaigns. 
The steps to quantify the CMF are 
%inspired from~\cite{Sheikh2016}.)
elaborated in Algorithm~\ref{algo:cmf-eval-strategy}. 
The number and sites of faults to be injected depends on the selected fault campaign as discussed in Section~\ref{sec:attack-model}.



\begin{algorithm}[ht]
\footnotesize
\caption{\bf: Common Mode Failure (CMF) Evaluation}
\label{algo:cmf-eval-strategy}
\begin{algorithmic} [1]
    \Require $R$ Replicas 
    \Require CMF Compute Engine~\ref{fig:cmf-compute-engine}
    \State {\bf$SIM$} : Simulation Count
    \State {\bf$F$} : Failure rate of the circuit
    \State {\bf$Rel$} : Reliability (\%) of the circuit
    \State {$\mathbf{V}$}: Randomly generated 100,000 test vectors
    \State {\bf$CMF_{OUT}$}: Instantaneous CMF detector output 
    \State {\bf$K$}   : Failure Count
    \State $K\gets0$
    \For{$(i = 1 \to SIM)$}
        \State Inject faults w.r.t. the {\it Error Campaign}
        \State Apply $\mathbf{V}$ to the circuit with faults injected        
        \State Compute CMF~(\ref{eqn:cmf-det}) and save results
        \For{$(j = 1 \to \mathbf{V})$}     
            \State {\bf if} ($CMF_{j} \ne 0$) {\bf then} increment $K$
        \EndFor
    \EndFor
    \State $F=\left(\frac{K}{SIM}\right)$
    \State $Rel(\%)=(1 - F)\times100$
\end{algorithmic}
\end{algorithm}
